Dynamical Disorder in the Mesophase Ferroelectric HdabcoClO4: A Machine-Learned Force Field Study

Hybrid molecular ferroelectrics with orientationally disordered mesophases offer significant promise as lead-free alternatives to traditional inorganic ferroelectrics owing to properties such as room temperature ferroelectricity, low-energy synthesis, malleability, and potential for multiaxial polarization. The ferroelectric molecular salt HdabcoClO4 is of particular interest due to its ultrafast ferroelectric room-temperature switching. However, so far, there is limited understanding of the nature of dynamical disorder arising in these compounds. Here, we employ the neural network NeuralIL to train a machine-learned force field (MLFF) with training data generated using density functional theory. The resulting MLFF-MD simulations exhibit phase transitions and thermal expansion in line with earlier reported experimental results, for both a low-temperature phasetransition coinciding with the orientational disorder of ClO4- molecules and the onset of rotation of Hdabco+ and ClO4- molecules in a high-temperature phase transition. We also find proton transfer even in the low-temperature phase, which increases with temperature and leads to associated proton disorder as well as the onset of disorder in the direction of the hydrogen-bonded chains.

==> defs.tex <==
\usepackage{color}
\usepackage{xcolor}
\usepackage{ulem}

\newcommand{\yambo}{\textsc{yambo}}
\newcommand{\qe}{\textsc{QuantumEspresso}}

\newcommand{\note}[1]{{\color{red}#1}}
%\renewcommand{\bibnumfmt}[1]{[#1] }



\newcommand{\editor}[2]{%
  \expandafter\newcommand\csname #1note\endcsname[1]{%
    \textcolor{#2}{(\textbf{#1:} \textit{##1})}}%
  \expandafter\newcommand\csname #1\endcsname[1]{%
    \textcolor{#2}{##1}}%
  \expandafter\newcommand\csname #1cancel\endcsname[1]{%
    \textcolor{#2}{\sout{##1}}}%
  \expandafter\newcommand\csname #1change\endcsname[2]{%
    \textcolor{#2}{\sout{##1} ##2}}%
  \newenvironment{#1text}{\color{#2}}{\color{black}}
}
\definecolor{Blu}{rgb}{0.00,0.00,1.00}
\definecolor{Red}{rgb}{1.00,0.00,0.00}
\definecolor{Cyan}{rgb}{0.00,0.50,0.50}
\definecolor{Green}{rgb}{0.00,0.70,0.00}

\editor{ES}{purple}
\editor{KB}{orange}

\input{defs.tex}


\renewcommand{\emph}{\textit}
\newcommand{\suppinfo}{Supplemental Material~\cite{supp-info}}
\newcommand{\ip}{\mathrm{Im}}
\newcommand{\rp}{\mathrm{Re}}

\newcommand{\reviewerA}[1]{\vspace{6pt}\noindent {\bf Reviewer 1: }{\it #1}}
\newcommand{\reviewerB}[1]{\vspace{6pt}\noindent {\bf Reviewer 2: }{\it #1}}
\newcommand{\reviewerC}[1]{\vspace{6pt}\noindent {\bf Reviewer 3: }{\it #1}}
\newcommand{\authors}[1]{\vspace{6pt}\noindent {\bf Authors Reply: } #1}
